BodyCam-VQA: Enhanced Body-Worn Camera Video Captioning via Multimodal Reasoning and Probe Question Generation

Police body-worn camera (BWC) footage has emerged as a critical aspect of law enforcement that ensures legal transparency, officer accountability, and the protection of civil rights. However, effectively processing this data remains a significant challenge due to its multimodal video format. BWC videos, in many cases, comprise chaotic scenes with low visual quality, rapid movement/interactions, and high-noise audio that make visual understanding a challenge for even SOTA multimodal models. Current Vision-Language Models (VLMs) frequently overlook critical forensic details, such as the presence of valuable evidence or the latent nuances of suspect-officer interactions, which are vital for fair legal outcomes and civilian/officer safety. To address these limitations, we propose an Adaptive Visual Question Answering (VQA) framework engineered for high-stakes law enforcement. Our framework employs a structured reasoning approach to extract fine-grained visual evidence that traditional captioning systems fail to capture. We experiment with multiple question generation models, including foundation models and fine-tuned open-weight models, to observe performance variation among question generation model implementations. Our results demonstrate that this VQA-driven architecture provides a more reliable, objective, and detailed record of enforcement events, ultimately serving as a powerful tool to protect both law enforcement officers and the public through AI-assisted forensic clarity.

==> header.tex <==

\newcommand{\draftonly}[1]{#1}
\newcommand{\draftcomment}[3]{\draftonly{\textcolor{#2}{{{[#1: #3]}}}}}
\newcommand{\mz}[1]{\draftcomment{Mengzhou}{purple}{#1}}
\newcommand{\sm}[1]{\draftcomment{Sadhika}{blue}{#1}}
\newcommand{\danqi}[1]{\draftcomment{Danqi}{orange}{#1}}
\newcommand{\suchin}[1]{\draftcomment{Suchin}{red}{#1}}

\newcommand{\cmark}{\checkmark}%
\newcommand{\xmark}{ }%
\newcommand{\flan}{\textsc{Flan V2}}
\newcommand{\cott}{\textsc{CoT}}
\newcommand{\dolly}{\textsc{Dolly}}
\newcommand{\hh}{\textsc{HH}}
\newcommand{\humaneval}{\textsc{HumanEval}}
\newcommand{\oasst}{\textsc{Open Assistant 1}}
\newcommand{\gsm}{\textsc{GSM}}
\newcommand{\shp}{\textsc{SHP}}
\newcommand{\se}{\textsc{SE}}
\newcommand{\gptalpaca}{\textsc{GPT4-Alpaca}}
\newcommand{\llamasmall}{\textsc{Llama-2-7B}}
\newcommand{\llamalarge}{\textsc{Llama-2-13B}}


\newcommand{\llamab}{\textsc{Llama-2-7B}}
\newcommand{\llamac}{\textsc{Llama-2-13B}}
\newcommand{\llamad}{\textsc{Llama-3-8B}}
\newcommand{\llamadinst}{\textsc{Llama-3-8B-Instruct}}
\newcommand{\llamae}{\textsc{Llama-3.1-8B}}
\newcommand{\llamaeinst}{\textsc{Llama-3.1-8B-Ins.}}
\newcommand{\mistralav}{\textsc{Mistral-7B-v0.1}}
\newcommand{\mistralavinst}{\textsc{Mistral-7B-Instruct-v0.1}}
\newcommand{\mistralb}{\textsc{Mistral-7B-v0.3}}
\newcommand{\mistralbinst}{\textsc{Mistral-7B-Ins.-v0.3}}





\newcommand{\mistral}{\textsc{Mistral-7B}}
\newcommand{\llamasmallchat}{\textsc{Llama-2-7B-Chat}}

\newcommand{\random}{Random}
\newcommand{\simdiv}{Sim + Div}
\newcommand{\simi}{Sim}
\newcommand{\less}{LESS}
\newcommand{\ours}{PU-ADKA}

\newcommand{\piref}{\pi_\text{ref}}


\definecolor{c1}{cmyk}{0,0.6175,0.8848,0.1490}
\definecolor{c2}{cmyk}{0.1127,0.6690,0,0.4431}
\definecolor{c3}{cmyk}{0.3081,0,0.7209,0.3255}
\definecolor{c4}{cmyk}{0.6765,0.2017,0,0.0667}
\definecolor{c5}{cmyk}{0,0.8765,0.7099,0.3647}

% Define colour boxes.
% Taken from https://arxiv.org/abs/2103.00453.
% \newtcbox{\hlprimarytab}{on line, rounded corners, box align=base, colback=c3!10,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newtcbox{\hlsecondarytab}{on line, box align=base, colback=red!10,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}

% \newtcbox{\flatbox}{on line, box align=base, colback=c4!10,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}

% Define up and down arrow commands.
\newcommand{\dashifted}{\raisebox{0.5\depth}{\tiny$\downarrow$}}
\newcommand{\uashifted}{\raisebox{0.5\depth}{\tiny$\uparrow$}}
\newcommand{\best}[1]{\textbf{\textcolor[RGB]{205,83,76}{#1}}}
\newcommand{\secondb}[1]{\textbf{\textcolor[RGB]{0,115,194}{#1}}}
% switched
\newcommand{\ua}[1]{{\small\hlprimarytab{\uashifted{#1}}}}
\newcommand{\da}[1]{{\small\hlsecondarytab{\dashifted{#1}}}}
\newcommand{\fa}[1]{{\small\flatbox{{#1}}}}
% switched

\newcommand{\uag}[1]{{\scriptsize\hlprimarytab{\uashifted{#1}}}}
\newcommand{\dab}[1]{{\scriptsize\hlsecondarytab{\dashifted{#1}}}}

\newcommand*{\TakeFourierOrnament}[1]{{%
\fontencoding{U}\fontfamily{futs}\selectfont\char#1}}
\newcommand*{\danger}{\TakeFourierOrnament{66}}

% \newcommand{\smallmodel}{\textsc{125m}}
% \newcommand{\medmodel}{\textsc{1.3b}}
% \newcommand{\largemodel}{\textsc{6.7b}}
% \newcommand{\xlmodel}{\textsc{13b}}
% \newcommand{\xxlmodel}{\textsc{30b}}
% \newcommand{\xxxlmodel}{\textsc{175b}}
% \newcommand{\ppl}{\textsc{ppl}}

\definecolor{gg}{HTML}{0F9D58}
\definecolor{rr}{HTML}{DB4437}
\definecolor{bb}{HTML}{4285F4}

% \newcommand{\flanv2}{\textsc{FLAN}}

\def\dsub{{\gD_{\text{train}}}}
\def\dfull{{\gD}}
\def\dval{{\gD_{\text{val}}}}
\def\dwarmup{{\gD_{\text{warmup}}}}
\newcommand{\valsub}[1]{{\gD_{\text{val}}^{(#1)}}}
\newcommand{\dtest}{\gD_{\text{test}}}
\def\numval{{m}}
\def\dim{{d}}
\newcommand{\grad}[2]{\nabla\ell(#1;#2)}
\newcommand{\loragrad}[2]{\hat\nabla\ell(#1;#2)}
\newcommand{\avggrad}[1]{\bar\nabla\ell(#1)}
\newcommand{\projgrad}[2]{\tilde\nabla\ell(#1;#2)}
\newcommand{\match}[2]{\gM(#1,#2)}
\newcommand{\diverse}[2]{\gK(#1,#2)}
\newcommand{\update}[2]{\Gamma(#1, #2)}
\newcommand{\loraupdate}[2]{\hat\Gamma(#1, #2)}
\newcommand{\approxupdate}[2]{\tilde\Gamma(#1, #2)}
\newcommand{\infadam}{{\textrm{Inf}_{\text{Adam}}}}
\newcommand{\infsgd}{{\textrm{Inf}_{\text{SGD}}}}

\newcommand{\std}[1]{\text{\scriptsize{(#1)}}}


